SpeedFolding: Learning Efficient Bimanual Folding of Garments

Folding garments reliably and efficiently is a long standing challenge in robotic manipulation due to the complex dynamics and high dimensional configuration space of garments. An intuitive approach is to initially manipulate the garment to a canonical smooth configuration before folding. In this work, we develop SpeedFolding, a reliable and efficient bimanual system, which given user-defined instructions as folding lines, manipulates an initially crumpled garment to (1) a smoothed and (2) a folded configuration. Our primary contribution is a novel neural network architecture that is able to predict pairs of gripper poses to parameterize a diverse set of bimanual action primitives. After learning from 4300 human-annotated and self-supervised actions, the robot is able to fold garments from a random initial configuration in under 120s on average with a success rate of 93%. Real-world experiments show that the system is able to generalize to unseen garments of different color, shape, and stiffness. While prior work achieved 3-6 Folds Per Hour (FPH), SpeedFolding achieves 30-40 FPH.

==> tables/time_benchmark.tex <==
\begin{table}[hb]
    \centering
    \caption{Average execution time for end-to-end folding}
\begin{tabular}{c|c|c}
    & Duration [\si{s}] & [\si{\%}] \\
\hline
    Camera Measurement & \num{14.6} & \\
    Robot Motions & \num{125.7} & \\
    Calculation & \num{13.2} & \\
\hline
    Total & \num{153.5} & - \\
\end{tabular}
    \label{tab:execution-time}
\end{table}
\begin{table}[hb]
    \centering
    \caption{Calculation performance BiMaMa-Net}
\begin{tabular}{c|c|c}
    & Duration [\si{ms}] & [\si{\%}] \\
\hline
    Pre-processing & \num{17.7 \pm 0.3} & \num{14.1 \pm 0.3} \\
    Classification Head & \num{14.07 \pm 0.02} & \num{11.17 \pm 0.02} \\
    Decoder & \num{16.25 \pm 0.04} & \num{12.90 \pm 0.03} \\
    Descriptor Sampling & \num{76.7 \pm 0.7} & \num{60.80 \pm 0.5} \\
    Descriptor Head & \num{0.89 \pm 0.01} & \num{0.71 \pm 0.01} \\
\hline
    Total & \num{126.0 \pm 0.9} & -
\end{tabular}
    \label{tab:execution-time}
\end{table}
